Contract-based Methodology for Developing Resilient Cyber-Infrastructure in the Industry 4.0 Era

As the industrial cyber-infrastructure become increasingly important to realise the objectives of Industry~4.0, the consequence of disruption due to internal or external faults become increasingly severe. Thus there is a need for a resilient infrastructure. In this paper, we propose a contract-based methodology where components across layers of the cyber-infrastructure are associated with contracts and a light-weight resilience manager. This allows the system to detect faults (contract violation monitored using observers) and react (change contracts dynamically) effectively.

==> content/02_outline.tex <==
%#######################################################################
	\section{Introduction \textbf{(1-Page)}}
	\begin{enumerate}
		\item Need for resiliency + CPS
		\item Proposed 3 layers (Application, Platforms, Physical system)
		\item Mmindmap from control and other related domains
		\item Our focus in on Platform layer
		\item Desired properties of resilient architecture
		\item Related work (briefly)
		\begin{itemize}
			\item Fault-tolerent work
			\item Self-Organising, Healing, xxxx
		\end{itemize}
		\item Research challenges (motivation)
	\end{enumerate}
	
	\section{Proposed Resilient Architecture for CPS \textbf{(1.5-Page)}}
	
	\begin{enumerate}
		\item Resiliency manager overview architecture (across 3~layers)
		\begin{itemize}
			\item steps: Monitor, Detect, Recovery plan, Learn.
			\item notion of evolution
			\item resilience state space (Normal, Degraded, Broken)
		\end{itemize}
		\item Resiliency metric (across 3~layers)
		\begin{itemize}
			\item Recovery time
			\item Quality of Service
			\item Cost
		\end{itemize}
		\item Detection techniques 
		\begin{itemize}
			\item Existing techniques (static, dynamic) 
			\item Need fo formal description
			\item Our approach to formal description of detection techniques
			\begin{itemize}
				\item templates using HA, TA, etc.
			\end{itemize}
		\end{itemize}
		\item Contract based evolution
		\begin{itemize}
			\item Contracts brief (2-way negotiation process)
			\item The flow diagram of an evolution.
		\end{itemize}
	\end{enumerate}
		
	\section{Example Scenarios from Smart Manufacturing \textbf{(1-Page)}}
	\begin{itemize}
		\item Scenario 1. Demonstrate
		\begin{itemize}
			\item Static fault detection
			\item Contract negotiation 
			\item Illustration of the evolution 
		\end{itemize}
		\item Scenario 2.  Demonstrate
		\begin{itemize}
			\item Dynamic fault detection
			\begin{itemize}
				\item Discretisation, Preservation of semantics
			\end{itemize}
			\item Contract negotiation 
			\item Illustration of the evolution 
		\end{itemize}
		
	\end{itemize}
	
	\section{Conclusions \& Future work \textbf{(0.25-Page)}}
\begin{itemize}
	\item Conclusions
	\item Future work
\end{itemize}
	
	\section{References \textbf{(0.25-Page)}}
	\cleardoublepage
%#######################################################################

==> figures/fig_componentStates.tex <==

\begin{tikzpicture}[scale=0.85, transform shape, yscale=0.8,
	node distance=5mm,
 	>=stealth,
 	block/.style = {,draw,minimum height=10mm,minimum width=28mm ,align=center},
 	every path/.style={->,ultra thick}
 	]

	\tikzstyle{block1}=[circle,draw=green!50,fill=green!20,ultra thick,minimum width=22mm,inner sep=0pt,align=center]
	\tikzstyle{block2}=[circle,draw=orange!50,fill=orange!20,ultra thick,minimum width=22mm,inner sep=0pt,align=center]
	\tikzstyle{block3}=[circle,draw=red!50,fill=red!20,ultra thick,minimum width=22mm,inner sep=0pt,align=center]
	
	\node [block1]						(norm) at  (2.6,3)	{Normal \\ State};
	\node [block2, left=of norm]  		(degraded) at (1.6,0.8) {Degraded \\ State};
	\node [block3, left=of degraded] 	(broken) at (-1.5,-0.5)	{Broken \\ State};
	
	%For boxes
	%\draw (norm.45)--($(norm.45)+(0.0,0.5)$)  -| node [shift={(-0.85,0.3)}]{Detect Failure} (degraded.135);
	%\draw (degraded.45)--($(degraded.45)+(0.0,0.5)$) -| node [shift={(-0.85,0.3)}]{Detect Failure} (broken.135);
	%Old Circle diagram
	%\path (norm.45) edge [bend left,align=center] node  [shift={(0.0,0.4)}]{Detect Failure} (degraded.135);
	%\path (degraded.45) edge [bend left,align=center] node  [shift={(0.0,0.4)}]{Detect Failure} (broken.135);
	%\path (broken.225) edge [bend left,align=center] node  [shift={(0.0,-0.4)}]{System Recovery} (degraded.-45);
	%\path (degraded.225) edge [bend left,align=center] node  [shift={(0.0,-0.4)}]{System Recovery} (norm.-45);
	\tikzset{every loop/.style={looseness=5}}
	
	\path (broken) edge [loop above,align=center,gray] node  {Unable to \\ recover} (broken);
	\path (norm) edge [loop above,align=center,gray] node  {Maintain} (norm);
	
	\path (norm) edge [bend left,align=center] node  [shift={(0.2,-0.4)},rotate=40]{Failure} (degraded);
	\path (degraded) edge [bend left,align=center] node  [shift={(-0.15,0.35)},rotate=40]{Recovery} (norm);
	
	
	\path (broken) edge [bend left,align=center] node  [shift={(0.0,0.4)},rotate=40]{Recovery} (degraded);
	\path (degraded) edge [bend left,align=center] node  [shift={(0.3,-0.2)},rotate=40]{Failure} (broken);
	
	
	
	\node [minimum width=0mm,inner sep=0pt](Ytop) at (-5,5) {};
	\node [minimum width=0mm,inner sep=0pt](origin1) at (-5,-3) {};
	\node [minimum width=0mm,inner sep=0pt](Xtop) at (4.0,-2) {};
	\node [minimum width=0mm,inner sep=0pt](origin2) at (-6,-2) {};
	
	\path (origin1) edge  node [shift={(-0.3,0.5)},rotate=90]{\Large Performance} (Ytop);
	\path (origin2) edge node  [shift={(0.0,-0.4)}]{\Large Resource Availability} (Xtop);
	
	\node[above=of Ytop, align = center, shift={(-0.5,-1.5)},inner sep=0pt,outer sep=0pt,rotate=90] (text0) {\small Acceptable};
	\node[above=of Ytop, align = center, shift={(-0.5,-6.5)},inner sep=0pt,outer sep=0pt,rotate=90] (text0) {\small Unacceptable};
	
	\node[below=of Xtop, align = center, shift={(-9,0)},inner sep=0pt,outer sep=0pt] (text0) {\small Low};
	\node[below=of Xtop, align = center, shift={(-1,0)},inner sep=0pt,outer sep=0pt] (text0) {\small Adequate};
	
	%\draw (broken)--($(broken.south)+(0.0,-0.5)$) -| node [shift={(0.85,-0.3)}]{System Recovery} (degraded.300);
	%\draw (degraded.225)--($(degraded.225)+(0.0,-0.5)$) -| node [shift={(0.85,-0.3)}]{ System Recovery} (norm.-45);


\end{tikzpicture}


==> figures/fig_contractBasedEvolution.tex <==
\begin{tikzpicture}[transform shape, scale=0.95 ]
[>=latex',every path/.style={->,ultra thick}]
%	\draw[step=1cm,gray!50,very thin] (-1.9,-10.9) grid (29.9,0.9);
	
	[node distance=0mm, >=latex',every path/.style={->,ultra thick}]
	
	\tikzstyle{blockABC1}=[rectangle,draw=blue!70,fill=blue!50,very thin,minimum width=7mm,inner sep=7pt,align=center]
	\tikzstyle{blockD1}=[rectangle,draw=blue!50,fill=blue!50,very thin,minimum width=15mm,inner sep=15pt,align=center]
	
	\tikzstyle{blockABC2}=[rectangle,draw=orange!50,fill=orange!50,ultra thick,minimum width=7mm,inner sep=7pt,align=center]
	\tikzstyle{blockD2}=[rectangle,draw=orange!50,fill=orange!50,ultra thick,minimum width=15mm,inner sep=15pt,align=center]

	\tikzstyle{nameless}=[draw,minimum height=10mm,minimum width=28mm ,align=center]
	
	\node [blockABC1, shift={(0,-0.5)}]			  	(A1)	{A};
	\node[above=of A1, align = center, shift={(4.3,-0.5)},inner sep=0pt,outer sep=0pt,] (text0) {\underline{\textbf{\Huge Contract Based Evolution}}};
	\node [blockABC1, right=of A1, shift={(-0.3,0)}]	(B1)	{B};
	\node [blockABC1, below=of B1, shift={(0.5,0.0)}]	(C1) {C};
	\node [blockD1,   below=of A1, shift={(0.2,0.0)}]	(D1) {D};
	\draw [<->, dotted, ultra thick](A1) -- (B1);
	\draw [<->, dotted, ultra thick](B1) -- (C1);
	\draw [<->, dotted, ultra thick](A1) -- (D1);
	
	\node [blockABC2, right=5.5cm of A1]  	(A2)	{A};
	\node [blockABC2, right=of A2, shift={(-0.3,0)}]			(B2)	{B};
	\node [blockABC2, below=of B2, shift={(0.5,0.0)}]	(C2) {C};
	\node [blockD2,   below=of A2, shift={(0.2,0.0)}]	(D2) {D};
	\draw [<->, dotted, ultra thick](A2) -- (B2);
	\draw [<->, dotted, ultra thick](B2) -- (C2);
	\draw [<->, dotted, ultra thick](A2) -- (D2);
	
	\node [blockABC1, below=4.2cm of A1]  	(A3)	{A};
	\node [blockABC1, right=of A3, shift={(-0.3,0)}]			(B3)	{B};
	\node [blockABC1, below=of B3, shift={(0.5,0.0)}]	(C3) {C};
	\node [blockD1,   below=of A3, shift={(0.2,0.0)}]	(D3) {D};
	\draw [<->, dotted, ultra thick](A3) -- (B3);
	\draw [<->, dotted, ultra thick](B3) -- (C3);
	\draw [<->, dotted, ultra thick](A3) -- (D3);
	
	\node [blockABC2, right=5.5cm of A3]  	(A4)	{A};
	\node [blockABC2, right=of A4, shift={(-0.3,0)}]			(B4)	{B};
	\node [blockABC2, below=of B4, shift={(0.5,0.0)}]	(C4) {C};
	\node [blockD2,   below=of A4, shift={(0.2,0.0)}]	(D4) {D};
	\draw [<->, dotted, ultra thick](A4) -- (B4);
	\draw [<->, dotted, ultra thick](B4) -- (C4);
	\draw [<->, dotted, ultra thick](A4) -- (D4);
	
	\begin{scope}[on background layer]
	\node [draw=black,fill=lime!20,inner sep=2pt,outer sep=0pt, fit=(A1)(B1)(C1)(D1)] [label={}] (ABox1){};
	\end{scope}
	\begin{scope}[on background layer]
	\node [draw=black,fill=lime!20,inner sep=2pt,outer sep=0pt, fit=(A2)(B2)(C2)(D2)] [label={}] (ABox2){};
	\end{scope}
	\begin{scope}[on background layer]
	\node [draw=black,fill=lime!20,inner sep=2pt,outer sep=0pt, fit=(A3)(B3)(C3)(D3)] [label={}] (ABox3){};
	\end{scope}
	\begin{scope}[on background layer]
	\node [draw=black,fill=lime!20,inner sep=2pt,outer sep=0pt, fit=(A4)(B4)(C4)(D4)] [label={}] (ABox4){};
	\end{scope}
	
	\tikzstyle{elli}=[ellipse,draw=black!45!green,fill=white!50,thick,minimum width=0mm,inner sep=3pt,align=center, ultra thick]
	
	\node [elli, right=of C1, shift={(-0.4,0)}]	(E1) {Tool 1 \\ \small Implement \\ \small Spec.};
	\draw [->, ultra thick] (ABox1) -- (E1);
	\draw [->, ultra thick] (E1) -- (ABox2);
	
	\node [elli, right=of C3, shift={(0,0.5)}]	(E2) {Tool 1};
	\draw [->, ultra thick] (ABox3) -- (E2);
	\draw [->, ultra thick] (E2) -- (ABox4);
	
	\tikzstyle{mon}=[rectangle,draw=blue!50,fill=cyan!70,thick,minimum width=0mm,inner sep=6pt,align=center]
	\tikzstyle{rec}=[rectangle,draw=blue!50,fill=blue!50,thick,minimum width=0mm,inner sep=6pt,align=center]
	
	\node [mon, right=of B2, shift={(1.5,-1)}]	(M1) {\Large Monitors \\ \small Detection \\ \small Techniques};
	\node [rec, below=of M1]	(R1) {\Large Recovery \\ \small Strategies};
	\draw [->, dotted, ultra thick](ABox2) -- node [shift={(-0.25,0.3)}]{Observers} (M1);
	\draw [->](M1) -- node [shift={(0.65,0.0)}]{Detect} (R1);
		
	\node [mon, right=of M1, shift={(2.5,0)}]	(M2) {\Large Monitors \\ \small Detection \\ \small Techniques};
	\node [rec, below=of M2]	(R2) {\Large Recovery \\ \small Strategies};
	
	\tikzstyle{elli2}=[ellipse,draw=black!45!green,fill=white!50,thick,minimum width=0mm,inner sep=3pt,align=center, ultra thick]
	\node [elli2, right=of M1, shift={(0,0)}]	(E3) {Tool 2};
	\node [elli2, right=of R1, shift={(0,0)}]	(E4) {Tool 3};
	\draw [->, ultra thick] (M2) -- (E3);
	\draw [->, ultra thick] (E3) -- (M1);
	\draw [->, ultra thick] (R2) -- (E4);
	\draw [->, ultra thick] (E4) -- (R1);
	\node[above=of M1, align = center, shift={(0,-0.8)},inner sep=0pt,outer sep=0pt,] (text1) {Resilience Manager \\ \textbf{(Synthesized)}};
	
	\begin{scope}[on background layer]
	\node [draw=black,fill=white!20,inner sep=15pt,outer sep=0pt,fit=(R1)(M1)(text1), ultra thick] [label={}] (ABox5) {};
	\end{scope}	

	\node[above=of M2, align = center, shift={(0,-0.8)},inner sep=0pt,outer sep=0pt,] (text2) {Resilience Manager \\ \textbf{(Specifications)}};		
	\begin{scope}[on background layer]
	\node [draw=black,fill=white!20,inner sep=15pt,outer sep=0pt,fit=(R2)(M2)(text2), ultra thick] [label={}] (ABox6) {};
	\end{scope}		
	

	\node[rectangle,draw=black!50,fill=gray!70,ultra thick,minimum width=10mm,inner sep=10pt,align=center,below=of R1,shift={(0,-2)}] (feasibility){Checks feasibility \\ of the strategy \\ (Cost, Resilience \\ metric, Contracts)};
	
	\node[above=of feasibility, align = center, shift={(0,-0.8)},inner sep=0pt,outer sep=0pt,] (Tool4) {\large Tool 4: \\ \small Resilience manager \\ \small(Global Level)};
	
	\begin{scope}[on background layer]
	\node [draw=black!30!green,ultra thick,fill=white!20,inner sep=10pt,outer sep=0pt,fit=(feasibility)(Tool4)] [label={}] (ABox7) {};
	\end{scope}

	\draw [->,red] (ABox7) -- node [shift={(-1.5,-0.3)}] {\textbf{Infeasible Strategy}}(R1);
	
	\node [blockABC1, right=of Tool4, shift={(1.2,-1)}]	  	(standaloneB)	{B};
	\node [blockABC1, right=of standaloneB]	(standaloneM)	{M};
	
	\newcommand{\Cross}{$\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.2ex, red] \draw (0,0) -- (1,1) (0,1) -- (1,0);}$}%
	
	\newcommand{\Checkmark}{$\color{black!40!green}\checkmark$}
	
	\node [above=of standaloneB, shift={(0,-1.1)}]	(cross)	{\Checkmark};
	\node [above=of standaloneM, shift={(0,-1.1)}]	(tick)	{\Cross};
	
	\begin{scope}[on background layer]
	\node [fill=gray!50,inner sep=10pt,outer sep=0pt,fit=(standaloneM)(standaloneB)] [label={Strategy X}] (ABox8) {};
	\end{scope}
	
	\draw [->, ultra thick] (ABox8.west) -- (ABox7);
	
	
	\draw [->, ultra thick,dotted] (R1) -- node [shift={(2.2,-0.2)}] {\textbf{Recovery Strategy}}(ABox8);
	
	\node[below=of standaloneB, align=center, shift={(0.7,0)},inner sep=0pt,outer sep=0pt,] (desire) {\large Desired \\ \large System-Level \\ \large Resilience};
	
	\draw [->, ultra thick] (desire) -- (ABox7);
	
	\node[regular polygon,regular polygon sides=5, fill=black!30!green!60, right=of desire, align=center, shift={(-0.75,0)},inner sep=10pt,outer sep=0pt,] (pentakun) {};
	
	\node [minimum width=0mm,inner sep=0pt,right of=desire, shift={(0,0)}]		(arrow1) {};
	\node [minimum width=0mm,inner sep=0pt,right of=desire]		(arrow2) {};
	\node [minimum width=0mm,inner sep=0pt,right of=desire]		(arrow3) {};
	\node [minimum width=0mm,inner sep=0pt,right of=desire]		(arrow4) {};
	\node [minimum width=0mm,inner sep=0pt,right of=desire]		(arrow5) {};
	
	\node [inner sep=0pt,above of=pentakun]								(arrow1partner) {};
	\node [inner sep=0pt, above right of =pentakun, shift={(0.3,-0.3)}]	(arrow2partner) {};
	\node [inner sep=0pt,below right of=pentakun, shift={(0.0,-0.2)}]		(arrow3partner) {};
	\node [inner sep=0pt,above left of=pentakun, shift={(-0.3,-0.3)}]		(arrow4partner) {};
	\node [inner sep=0pt,below left of=pentakun, shift={(0,-0.2)}]		(arrow5partner) {};
	
	\draw [->, ultra thick] (pentakun.center) -- (arrow1partner);
	\draw [->, ultra thick] (pentakun.center) -- (arrow2partner);
	\draw [->, ultra thick] (pentakun.center) -- (arrow3partner);
	\draw [->, ultra thick] (pentakun.center) -- (arrow4partner);
	\draw [->, ultra thick] (pentakun.center) -- (arrow5partner);
	
	\draw [->,ultra thick,black!55!green] ( ABox7.225) -| ($(ABox3.south)+(0,-0.3)$) -- node [shift={(5.0,-0.2)}]{\textbf{\large Feasible Strategy}} (ABox3.south);
	
	
%	\draw (norm)--($(norm.north)+(0.0,0.5)$)  -| node [shift={(-0.85,0.3)}]{Detect Failure} (degraded.135);
	
	
	
	
	
		
	
	
\end{tikzpicture}




==> figures/fig_resilientArchitecture.tex <==
\begin{tikzpicture}[transform shape, scale=0.8 ]
	[node distance=5mm, >=latex',
	every path/.style={->,ultra thick}]
	\tikzstyle{block2}=[rectangle,draw=red!50,fill=red!20,ultra thick,minimum width=20mm,inner sep=50pt,align=center]
	\tikzstyle{block}=[draw,minimum height=10mm,minimum width=28mm ,align=center]
	
	
	%Resilience manager
	\node [block]                      (gather)     {Gather \\ Monitor Data};
	\node [block, right=of gather]      (check)   {Check};
	\node [block, right=of check] (recoverStrategy) {Recover Strategy};
	\node [block, right=of recoverStrategy] (learning) {Learning};
	\draw (gather) -- (check);
	\draw (check) to (recoverStrategy);
	\draw[<->] (recoverStrategy) to (learning);
	\draw (learning)--($(learning.north)+(0,0.5)$) -| (gather);
	\draw (recoverStrategy)--($(recoverStrategy.north)+(0,0.5)$) -| (gather);
	
	\begin{scope}[on background layer]
	\node [fill=lime!20,inner sep=33pt,outer sep=0pt, fit=(gather) (check) (recoverStrategy)
	(learning)] [label={Resilience Manager}] (hello){};
	\end{scope}
	
	\begin{scope}[on background layer]
	\node [draw,dashed,fill=yellow!20,inner sep=8pt,outer sep=0pt,fit=(gather) (check)][label={}] (monitored){};
	\end{scope}
	
	
	
	%System
	\tikzstyle{edge}=[rectangle,draw=blue!50,fill=blue!20,thick,minimum width=7mm,,align=center]
	
	\tikzstyle{sen}=[diamond,draw=violet!50,fill=violet!20,ultra thick,minimum width=7mm,align=center]
	\tikzstyle{act}=[circle,draw=green!50,fill=green!20,thick,minimum width=9mm,,align=center]
	%edges
	\node [block2, left=3.2cm of gather] (system) {System};
	\node [edge, left=-0.4cm of system] (e1) {E};
	\node [edge, above=of e1] (e2) {E};
	\node [edge, below=of e1] (e3) {E};
	\node [edge, right=-0.4cm of system] (e4) {E};
	\node [edge, above=of e4] (e5) {E};
	\node [edge, below=of e4] (e6) {E};
	%sensors and actuators
	\node [sen, left=of e1] (s1) {S};
	\node [sen, left=of e2] (s2) {S};
	\node [act, left=of e3] (a1) {A};
	\node [act, right=of e4] (a2) {A};
	\node [act, right=of e5] (a3) {A};
	\node [sen, right=of e6] (s3) {S};
	\draw [<->](s1) -- (e1);
	\draw [<->](s2) -- (e2);
	\draw [<->](s3) -- (e6);
	\draw [<->](a1) -- (e3);
	\draw [<->](a2) -- (e4);
	\draw [<->](a3) -- (e5);
	
	\path (hello.165) edge [bend right,<->,align=center] node {} (system);
	
	
	%Policies
	\tikzstyle{block3}=[rectangle,draw=orange!50,fill=orange!20,ultra thick,minimum width=60mm,inner sep=30pt,align=center]
	
	\tikzstyle{block4}=[rectangle,draw=black!50,fill=black!20,ultra thick,minimum width=0mm,inner sep=5pt,align=center]
	
	\node [block3, below=2cm of recoverStrategy] (policy) [label={[shift={(-2.0,0.0)}]Policies}]{};
	
	\node [block4, below=2.5cm of recoverStrategy, shift={(-2.0,0.0)}] (p1) {Action};
	\node [block4, right=of p1, shift={(-0.5,0.0)}] (p2) {Action};
	\node [block4, right=of p2, shift={(-0.5,0.0)}] (p3) {Action};
	
	\draw [densely dotted,-](p1) -- (p2);
	\draw [densely dotted,-](p2) -- (p3);
	
	%Monitors
	\tikzstyle{block5}=[rectangle,draw=cyan!50,fill=cyan!20,ultra thick,minimum width=48mm,inner sep=45pt,align=center]
	
	\tikzstyle{block6}=[rectangle,draw=black!50,fill=black!20,ultra thick,minimum width=0mm,inner sep=18pt,align=center]
	
	\tikzstyle{edge2}=[circle,draw=violet!50,fill=violet!20,thick,minimum width=5mm,,align=center]
	
	\node [block5, below=1.5cm of monitored, shift={(-1.0,0.0)}] (monitor) [label={[shift={(-1.0,0.0)}]Monitors}]{};
	
	%\node [block6, below=1.8cm of monitored, shift={(-2.6,0.0)}] (m1) {M};
	%\node [block6, right=of m1] (m2) {M};
	%\node [block6, right=of m2] (m3) {M};
	
	\node [block6, below=1.8cm of monitored, shift={(-1.8,0.0)}] (inter) {Interface};
	
	\node [edge2, right=of inter, shift={(-0.1,0.5)}] (ed1) {};
	\node [edge2, below=of ed1, shift={(0.6,0.1)}] (ed2) {};
	\node [edge2, below=of ed1, shift={(0,-0.8)}] (ed3) {};
	
	\draw [<->](ed1) -- (ed2);
	\draw [<->](ed2) -- (ed3);
	\draw [<->](ed3) -- (ed1);
	
	\path (ed1.north) edge [bend right=30pt,-,dashed,align=center] node {} (inter);
	\path (ed3.195) edge [bend left,-,dashed,align=center] node {} (inter);
	
	

\end{tikzpicture}  

==> tables/tab_detectStratagies.tex <==

\begin{table*}[tbhp]
	\centering
	\caption{Comparison of existing failure detection techniques}
\begin{tabular}{|p{3cm}|c|p{1.2cm}|c|p{5cm}|}
\hline 
\textbf{Detection Technique} & 
\textbf{Domain} &  
\textbf{Layer(s)}  &  
\textbf{Classification}& 
\textbf{Description} 
\\\hline
Sequence number~\cite{Kanodia1974}
&  Fault-tolerance
&  SN
&  \mDTab
&  Missing number in the sequence $(1,2,4,5)\to$ message $3$ not received. 
\\ \hline 
Time-outs or heartbeats
&  Fault-tolerance
&  SN
&  \mDTab
&  Message should have arrived by now (upper time bound).
\\ \hline
Replication
&  Fault-tolerance
& SNL
&  \mDTmm
&  Compare data for equality
\\ \hline
Sequence-Based Fault Detection (SBFD)~\cite{Kamal2014}
&  Fault-tolerance
& N
&  \mDTmm
&  Given a network topology (dynamic or static) and the packet path, receivers can identify faulty nodes.
\\ \hline
Model based reasoning (static)~\cite{Isermann2005}
&  Fault-tolerance
&  SNL
&  \mDTmm
&  Algebraic equation e.g, $x+y \leq 10$, Logic e.g., \texttt{IF (condition) THEN <conclusion>}
\\ \hline
Model based reasoning (dynamic)~\cite{Isermann2005}
&  Fault-tolerance
&  SNL
&  \mDTmm
&  Time dependent. \acp{ODE} e.g, $\frac{dx}{dt} \leq 0.7$
\\ \hline
Model based reasoning (patterns, without prior knowledge)~\cite{Isermann2005}
&  Fault-tolerance
&  SNL
&  \mDTmm
& No prior knowledge is available. Statistical analysis for probabilistic fault detection
\\ \hline
&  
& 
&  
&  
\\ \hline
&  
& 
&  
&  
\\ \hline
&  
& 
&  
&  
\\ \hline
\end{tabular}
\end{table*} 

==> tables/tab_recoveryStratagies.tex <==

\begin{table*}[tbhp]
	\centering
	\caption{Comparison of existing recovery strategies}
\begin{tabular}{|c|c|c|c|c|}
\hline 
\textbf{Recovery strategy} &  &  &  & \textbf{Description} \\
 \hline
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
&  &  &  &  \\ 
\hline 
\end{tabular}
\end{table*} 

==> tables/tab_resilientArchs.tex <==

\begin{table*}[tbhp]
	\centering
	\caption{Comparison of existing resilient architectures}

\begin{tabular}{|c|c|c|c|c|c|c|}
	\hline
	
	& \multirow{ 2}{*}{\textbf{Architecture} }
	& \multicolumn{4}{c|}{\textbf{Features}} 
	& \multirow{ 2}{*}{\textbf{Target} } \\ 
	\cline{3-6}
	&
	&  \textbf{data collection}
	&  \textbf{fault detection}
	&  \textbf{fault containment}
	&  \textbf{adapt/reconfigure}
	&
	\\ 
	\cline{1-7}
	\multirow{5}{*}{\rotatebox[]{90}{\textbf{Self-Adaptive}} }
	&Kinesthetics eXtream~\cite{Valetto2002} 
	&  using probes and gauges
	&  Complex event processing~\cite{Luckham1998} 
	&  
	&  using effectors
	&  
	\\ 
	\cline{2-7}
	&&  &  &  &  &  \\ 
	
	\cline{2-7}
	&&  &  &  &  &  \\ 
	
	\cline{2-7} 
	&&  &  &  &  &  \\ 
	
	\cline{2-7} 
	&&  &  &  &  &  \\ 
	\hline 
\end{tabular} 
\end{table*}
